Towards Understanding and Mitigating Audio Adversarial Examples for Speaker Recognition

Speaker recognition systems (SRSs) have recently been shown to be vulnerable to adversarial attacks, raising significant security concerns. In this work, we systematically investigate transformation and adversarial training based defenses for securing SRSs. According to the characteristic of SRSs, we present 22 diverse transformations and thoroughly evaluate them using 7 recent promising adversarial attacks (4 white-box and 3 black-box) on speaker recognition. With careful regard for best practices in defense evaluations, we analyze the strength of transformations to withstand adaptive attacks. We also evaluate and understand their effectiveness against adaptive attacks when combined with adversarial training. Our study provides lots of useful insights and findings, many of them are new or inconsistent with the conclusions in the image and speech recognition domains, e.g., variable and constant bit rate speech compressions have different performance, and some non-differentiable transformations remain effective against current promising evasion techniques which often work well in the image domain. We demonstrate that the proposed novel feature-level transformation combined with adversarial training is rather effective compared to the sole adversarial training in a complete white-box setting, e.g., increasing the accuracy by 13.62% and attack cost by two orders of magnitude, while other transformations do not necessarily improve the overall defense capability. This work sheds further light on the research directions in this field. We also release our evaluation platform SPEAKERGUARD to foster further research.

==> SRSs.tex <==
% \section{Background}\label{sec:background}\vspace*{-1mm}


\section{Speaker Recognition Systems}\label{sec:background}%\vspace*{-1mm}

% In this section, we introduce the preliminaries of mainstream and state-of-the-art SRSs and their recognition tasks.
In this section, we introduce the preliminaries of mainstream and state-of-the-art SRSs
and their recognition tasks as well as text dependency.
%\sen{Why does title use voice print recognition?} \chengk{Answer: We can discuss the title and whether to use voiceprint recognition or speaker recognition later.}

%\subsection{Speaker Recognition Systems}


%\noindent {\bf Overview of SRSs.}
%\vspace*{-1mm}
\subsection{Overview of Speaker Recognition}%\vspace*{-1mm}
Modern and state-of-the-art SRSs use speaker embedding~\cite{wang2020simulation} to represent
acoustic characteristics of speakers as fixed-dimensional vectors.
The typical
speaker embedding is identity-vector (ivector)~\cite{DehakDKBOD09} based on the Gaussian Mixture Model (GMM)~\cite{ReynoldsR95,reynolds2000speaker}.
Recently, deep embedding was also proposed to compete with ivector.
It first uses deep learning to train a deep neural network, then
extracts
% acoustic characteristics
speaker characteristics
from the deep neural network
and often presents
% acoustic characteristics
speaker characteristics
as dvector~\cite{variani2014deep} or xvector~\cite{snyder2018x}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{fig/overview-SRSs-2}
    \vspace*{-2mm}
    \caption{Architecture of SRSs.}
    \label{fig:typical-SRSs}\vspace*{-4mm}
\end{figure}

A generic architecture of SRSs is shown in \figurename~\ref{fig:typical-SRSs}, consisting of three phases: training, enrollment, and recognition phases.
In the training phase, a background model is trained using tens of thousands of voices from thousands of training speakers,
representing the speaker-independent distribution of voice features.
%
In the enrollment phase, the background model maps the voice uttered by each enrolling speaker to an \emph{enrollment embedding},
regarded as the unique identity of the enrolling speaker.
%
In the recognition phase, given a voice of an unknown speaker, the \emph{voice embedding} is extracted from the background model
for scoring. The scoring module measures the similarity between the \emph{enrollment embedding} and \emph{voice embedding} based on which the result is produced by the decision module.
There are two typical scoring approaches: Probabilistic Linear Discriminant Analysis (PLDA)~\cite{nandwana2019analysis}
and COSine Similarity (COSS)~\cite{dehak2010cosine}.
The former approach works well in most situations, but needs to be trained using voices~\cite{wang2020simulation}.
The latter approach is a reasonable substitution of PLDA
% without training.
which does not need to be trained.
 
% \chengk{TO DO: If we do not extend adversarial training to enrollment-type system, we do not use cosine distance, so the detail of scoring module can be removed.}
% The scoring module is commonly based on probabilistic linear discriminant analysis (PLDA)~\cite{nandwana2019analysis} or cosine distance~\cite{dehak2010cosine}.

% Note that usually after training, the embeddings are extracted from some intermediate layer of the embedding network and the subsequent layers (including \texttt{softmax} layer) layers are removed.

The feature extraction module converts raw speech signals to acoustic features
% (as vectors)
carrying characteristics of the raw signals.
Common feature extraction algorithms include Mel-Frequency Cepstral Coefficients (MFCC)~\cite{muda2010voice} and
Perceptual Linear Predictive (PLP)~\cite{hermansky1990perceptual}.

%\noindent {\bf Speaker recognition tasks.}
%\vspace*{-2mm}
\subsection{Recognition Tasks}\label{sec:SR-task}%\vspace*{-1mm}
There are three main tasks in SR: close-set identification (CSI), speaker verification (SV), and open-set identification (OSI).
CSI identifies a speaker from
% a set of
a group of
% enrolled speakers,
candidate speakers,
which is a multi-class classification problem.
SV verifies if an input voice is uttered by the unique enrolled speaker, according to a preset threshold, where
the input voice may be rejected by regarding the speaker as an imposter.
%OSI can be seen as a combination of CSI and SV.
OSI utilizes the scores and a preset threshold to identify which enrolled speaker utters the input voice.
If the highest score is less than the threshold, the input voice is rejected by regarding the speaker as an imposter.
Furthermore, CSI could be classified into two sub-tasks:
CSI with enrollment (CSI-E) and  CSI without enrollment (CSI-NE).
CSI-E exactly follows the above description.
In contrast, CSI-NE does not have the enrollment phase
and the background model is directly utilized to identify speakers.
Thus, ideally,  %the system can be seen as an end-to-end one and
    % recognized speakers should be involved in the training phase.
   a recognized speaker in CSI-NE task is involved in the training phase,
   while a recognized speaker in CSI-E task should have enrolled in the enrollment phase but may not be involved in the training phase.

We remark that the enrollment phase and scoring module are rarely used
in image and speech recognition systems.
% \chengk{Formally speaking,
% a SR model can be denoted by
% % ${\tt SR}_{\text{task}}(x):\mathcal{X} \rightarrow \mathcal{Y}$,
% ${D}(x):\mathcal{X} \rightarrow \mathcal{Y}$,
% where
% % $x\in\mathcal{X}\subset \mathbb{R}^d$ s
% $x\in\mathcal{X}$
% is the input voice, and $\mathcal{Y}$ the
% % space of decision.
% decision space.
% For CSI task, $\mathcal{Y}=\{1,2,\cdots,M\}$ with $M\ (M>1)$ being the number of candidate speakers. For SV task, $\mathcal{Y}=\{{\tt accept}, {\tt reject}\}$. For OSI task, $\mathcal{Y}=\{1,2,\cdots,M,{\tt reject}\}$.}

% \subsection{Text Dependency}
% % SRSs can be either text-dependent, where cooperative speakers are required to utter one of pre-defined sentences,
% % or text-independent, where the speakers are allowed to speak anything.
% SRSs can be either text-dependent, where cooperative speakers must use the same passphrase during enrollment and recognition,
% or text-independent, where the speakers can utter arbitrary phrases.
% The former achieves high accuracy on short utterances,
% but always requires a large amount utterances containing the same phrase,
% thus it is limited to the SV task.
% The latter may require longer utterances to achieve high accuracy,
% but practically it is more flexible and suits for all recognition tasks~\cite{Homayoon11}.
% Therefore, in this work, we mainly perform our empirical study on text-independent SRSs.
% Temporal dependency is critical for reducing recognition error rate in text-dependent SRSs~\cite{temporal-text-dependent},
% while is unimportant for text-independent SRSs~\cite{speech-processing-book}.

% It is unknown whether the subject presented to the biometric system for recognition has enrolled in the system or not. Therefore, the system needs to decide whether to reject or recognize him as one of the enrolled subject. It is the opposite of Closed-Set Identification.
%
% The main body of this paper concentrates on CSI task, and the other two tasks are discussed in section~\ref{sec:extend-adver-train}.
%To diversify the experiment, we take into account two types of CSI task:
%\begin{itemize}
%    \item CSI without enrollment (CSI-NE): In this task,
%    % the enrollment phase is not involved in the architecture in \figurename~\ref{fig:typical-SRSs}
%    the enrollment phase in \figurename~\ref{fig:typical-SRSs} will not be executed
%    and the background model is directly utilized to identify speakers.
%    Ideally, in this setting, %the system can be seen as an end-to-end one and
%    % recognized speakers should be involved in the training phase.
%   each recognized speaker is involved in the training phase.
%    % The set of speakers to be identified in the recognition phase is exactly the set of training speakers in the training phase.
%    CSI-NE is similar to image classification.
%    \item CSI with enrollment (CSI-E): CSI-E exactly follows the architecture in \figurename~\ref{fig:typical-SRSs},
%     where the background model, representing the speaker-independent
%distribution of voice feature, is used to map the voice uttered by each enroll speaker to an enrollment embedding.
%% Recognized speakers should be enrolled in enrollment phases but are not necessarily involved in the training phase.
%Ideally, a recognized speaker should have enrolled in the enrollment phase but may not involved in the training phase.
%    % \sen{Why just mention the fig to introduce the current type?}
%\end{itemize}


==> evaluation-attack.tex <==


\begin{table}[t]
    \centering
    % \caption{The effectiveness and stealthiness of attacks.}
    \caption{Effectiveness and stealthiness of untargeted attacks.}
\resizebox{0.45\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \hline
      \multicolumn{2}{c|}{\multirow{2}{*}{\bf Attack}} & {\bf Effectiveness} & \multicolumn{3}{c}{\bf Stealthiness} \\ \cline{3-6}
       \multicolumn{2}{c|}{} & {\bf ASR} & \bm{$L_2$} & {\bf SNR} & {\bf PESQ} \\ \hline
       \multicolumn{2}{c|}{\bf FGSM} & 57.7\% & 0.537 & 28.53 & 2.23 \\ \hline
       \multirow{6}{*}{\bf {PGD-$\mathbf{x}$}} & $\mathbf{x}${\bf =10} & 100\% & 0.330 & 32.77 & 2.85 \\ \cline{2-6}
       & $\mathbf{x}${\bf =20} & 100\% & 0.378 & 31.57 & 2.72 \\ \cline{2-6}
       & $\mathbf{x}${\bf =30} & 100\% & 0.385 & 31.42 & 2.70 \\ \cline{2-6}
       & $\mathbf{x}${\bf =40} & 100\% & 0.384 & 31.45 & 2.71 \\ \cline{2-6}
       & $\mathbf{x}${\bf =50} & 100\% & 0.390 & 31.31 & 2.69 \\ \cline{2-6}
       & $\mathbf{x}${\bf =100} & 100\% & 0.391 & 31.29 & 2.70 \\ \hline
       \multicolumn{2}{c|}{\bf CW\bm{$\infty$}-0} & 100\% & 0.378 & 31.57 & 2.72 \\ \hline
       \multirow{5}{*}{\bf CW$_2$-$\kappa$} & $\mathbf{\kappa}${\bf =0} & 93.5\% & 0.041 & 52.99 & 4.24 \\\cline{2-6}
       & $\mathbf{\kappa}${\bf =5} & 100\% & 0.058 & 49.73 & 4.10 \\ \cline{2-6}
       & $\mathbf{\kappa}${\bf =10} & 100\% & 0.078 & 47.09 & 3.95\\ \cline{2-6}
    & $\mathbf{\kappa}${\bf =20} & 100\% & 0.131 & 42.14 & 3.60 \\ \cline{2-6}
      & $\mathbf{\kappa}${\bf =50} & 100\% & 0.476 & 30.44 & 2.46 \\ \hline
      \multirow{2}{*}{\bf FAKEBOB}&\#Iter=1000 & 99.7\% & 0.397 & 31.12  & 2.67  \\ \cline{2-6}
     &\#Iter=200& 80.2\% & 0.383 & 31.40 & 2.71 \\ \hline
    % \multicolumn{2}{c|}{\bf FAKEBOB} &  &  &  &  \\ \hline
    \end{tabular}}
    \label{tab:evaluate-atatck} \vspace*{-2mm}
\end{table}

\subsection{Evaluation of Attacks}\label{sec:evaluate-attack}
\noindent{\bf Experimental Setup}.
We consider the ivector-PLDA model for the CSI-E task which is enrolled with 10 speakers using Spk$_{10}$-enroll. %, forming a speaker group.
We use Spk$_{10}$-test to test the model, resulting in 99.8\% accuracy on benign examples.
We will also use Spk$_{10}$-test to generate adversarial examples.
% \chengk{TO DO: After I have finished targeted attack experiment, we should tell how to specify targeted label for targeted attack here.}
The target label of targeted attack for each voice is randomly chosen among the labels except the ground truth.

% \ling{00: anything needed to set up or mention for FGSM?}
We use 10, 20, 30, 40, 50 and 100 steps for PGD, and 30 steps for CW$_{\bm{\infty}}$,
with step size $\alpha=\frac{\epsilon}{5}=0.0004$.
The step size of FGSM is $\epsilon=0.002$.
For CW$_2$, we use 9 binary search steps to minimize adversarial perturbations, run 900-9000 iterations to converge, and vary the parameter $\kappa$ from 0, 5, 10, 20 to 50.
% We use the default parameters of FAKEBOB since our target model is exactly the one in \cite{chen2019real}. The iteration limit is 1000 and the samples\_per\_draw of NES $m$ is 50.
For FAKEBOB, we set the iteration limit (denoted by \#Iter) to 1000 and samples\_per\_draw $m$ of NES to $50$, the same as~\cite{chen2019real}.
We set $\kappa=0.5$ for FAKEBOB so that adversarial voices remain adversarial after stored
back into the 16-bit PCM form.
We do not study  SirenAttack as it is less effective than FAKEBOB~\cite{chen2019real}.
% \chengk{TO DO: Loss function for FGSM, PGD, CW$_2$. Use a Table ?}
% \ling{00: remember to mention the evaluation metrics such as ASR if not mentioned before.}


%%%%%%%%%%%% remove UTR
\begin{table}[t]
    \centering
    % \caption{The effectiveness and stealthiness of attacks.}
    \caption{Effectiveness and stealthiness of targeted attacks.}
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \hline
      \multicolumn{2}{c|}{\multirow{2}{*}{\bf Attack}} & {\bf Effectiveness} & \multicolumn{3}{c}{\bf Stealthiness} \\ \cline{3-6}
       \multicolumn{2}{c|}{} & {\bf ASR} & \bm{$L_2$} & {\bf SNR} & {\bf PESQ} \\ \hline
       \multicolumn{2}{c|}{\bf FGSM} & 40.2\% & 0.537 & 28.53 & 2.23 \\ \hline
       \multirow{6}{*}{\bf {PGD-$\mathbf{x}$}} & $\mathbf{x}${\bf =10} & 99.7\% & 0.317 & 33.12 & 2.87 \\ \cline{2-6}
       & $\mathbf{x}${\bf =20} & 99.7\% & 0.356 & 32.10 & 2.77 \\ \cline{2-6}
       & $\mathbf{x}${\bf =30} & 99.9\% & 0.368 & 31.82 & 2.75 \\ \cline{2-6}
       & $\mathbf{x}${\bf =40} & 99.9\% & 0.373 & 31.69 & 2.74 \\ \cline{2-6}
       & $\mathbf{x}${\bf =50} & 100\% & 0.376 & 31.63 & 2.73 \\ \cline{2-6}
       & $\mathbf{x}${\bf =100} & 100\% & 0.380 & 31.53 & 2.72 \\ \hline
       \multicolumn{2}{c|}{\bf CW\bm{$\infty$}-0} & 100\% & 0.369 & 31.79 & 2.74 \\ \hline
       \multirow{5}{*}{\bf CW$_2$-$\kappa$}  & $\mathbf{\kappa}${\bf =0} & 96.9\% & 0.083 & 46.93 & 3.92 \\ \cline{2-6}
       & $\mathbf{\kappa}${\bf =5} & 100\% & 0.105 & 44.53 & 3.77 \\ \cline{2-6}
       & $\mathbf{\kappa}${\bf =10} & 100\% & 0.139 & 41.79 & 3.57 \\ \cline{2-6}
    & $\mathbf{\kappa}${\bf =20} &  100\% & 0.290 & 35.03 & 2.94 \\ \cline{2-6}
      & $\mathbf{\kappa}${\bf =50} &  100\% &  1.714 & 18.91 & 1.51 \\ \hline
      \multirow{2}{*}{\bf FAKEBOB}&\#Iter=1000 & 95.2\% & 0.383 & 31.44 & 2.70  \\ \cline{2-6}
     &\#Iter=200& 51.5\% & 0.378 & 31.60 & 2.72 \\ \hline
    \end{tabular}
    }
    \label{tab:evaluate-atatck-target} \vspace*{-2mm}
\end{table}
%\subsubsection{Experimental Results}\label{sec:evaluate-attack-result}
% The result of untargeted attack is shown in \tablename~\ref{tab:evaluate-atatck}, and the result of targeted attack is shown in \tablename~\ref{tab:evaluate-atatck-target}.
%The result of untargeted attack is shown in \tablename~\ref{tab:evaluate-atatck}.
{\tablename~\ref{tab:evaluate-atatck} and \tablename~\ref{tab:evaluate-atatck-target} show the results of untargeted and target attacks, respectively.}
%\sen{Due to the iteration limit, I am a little confused about the results of these two tables, because the the results are inconsistent with the oakland paper. Do we need to provide some claims in the setup?}
%\fu{Redo the experiments on FAKEBOB}

% \noindent {\bf Effectiveness.}
% Among $L_\infty$ norm attacks, FGSM is the least effective with only $53.5\%$ ASR. This is because FGSM is single-step attack. PGD and CW$_{\bm{\infty}}$ are the most powerful which reduces model accuracy on adversarial voices to 0\%. FAKEBOB attack is about 20\% less effective than PGD and CW$_{\bm{\infty}}$ since it exploits estimated gradient which may not be accurate enough. The effectiveness of FAKEBOB attack can be improved by increasing samples\_per\_draw $m$ and iteration limit. When $\kappa<20$, the ASR of CW$_2$ is less than 100\%. However, we exam the procedure of computing adversarial perturbation and find that even when $\kappa=0$, CW$2$ achieves 100\% ASR in float domain. This demonstrates that CW$2$ with low confidence suffers from severe discretization problem~\cite{bu2019taking}, i.e., successfully crafted adversarial examples in real continuous domain become benign once transformed back into concrete integer domain. The reason is that CW$_2$ seeks for minimal perturbation which is so minor that can be easily disrupted by the transformation between continuous and discrete domain. To overcome this problem, we need to increase the $\kappa$ of CW$_2$. When $\kappa=20,50$, CW$_2$ achieves 100\% ASR.
\smallskip\noindent {\bf Effectiveness.}
We can observe from \tablename~\ref{tab:evaluate-atatck} that
FGSM is less effective than others, with only $57.7\%$ ASR. This is because FGSM is a single-step attack.
PGD, CW$_{\bm{\infty}}$ and FAKEBOB are the most powerful attacks whose ASR is close to 100\% ASR.
When $\kappa=0$, the ASR of CW$_2$ is 93.5\%.
With the increase of $\kappa$, CW$_2$ achieves 100\% ASR.

From \tablename~\ref{tab:evaluate-atatck-target}, we can observe that
FGSM, PGD-10, PGD-20, PGD-30, PGD-40, and FAKEBOB become slightly less effective
for targeted attack, while the others have the same ASR
for both targeted and untargeted attacks.


We remark that CW$_2$-0 achieved 100\% ASR before storing the adversarial examples back into the 16-bit PCM form.
This means that CW$_2$-0 suffers from the discretization problem~\cite{bu2019taking}.
This is because  CW$_2$ seeks for minimal adversarial perturbations which are too small to be easily disrupted when $\kappa=0$.
This problem is avoided by increasing $\kappa$.
%{the $\kappa$ of CW$_2$ needs to be increased. As expected, }
%when $\kappa=5$,

We also report the results of FAKEBOB with 200 iteration limit.
It becomes 19.5\% less effective for untargeted attack and 43.7\% less effective for targeted attack.
FAKEBOB with 200 iteration limit will be used to evaluate defenses
against untargeted attacks in consideration of the experiment effort.

\smallskip\noindent {\bf Stealthiness.}
From \tablename~\ref{tab:evaluate-atatck}, we observe that FAKEBOB, PGD and CW$_{\bm{\infty}}$  achieve comparable
results in terms of $L_2$ norm, SNR, and PESQ.
Unsurprisingly, adversarial voices crafted by FGSM are more perceptible than others.
When $\kappa\leq 20$, CW$_2$ achieves the best imperceptibility with at least 42 dB SNR and 3.6 PESQ.
This is because CW$_2$ uses a binary search to minimize perturbations. However, with the increase of $\kappa$, CW$_2$ becomes significantly more perceptible.
% \ling{anything to mention about PESQ? otherwise what is the intention for putting it here? try to dig out more findings from the table as this section is a kind of empirical study.}

From \tablename~\ref{tab:evaluate-atatck-target}, we can observe that
FGSM, PGD-10, PGD-20, PGD-30, PGD-40, and FAKEBOB for targeted attack
achieve similar stealthiness as for untargeted attack.
% This is not surprisingly since targeted attack is more challenging than untargeted attack for adversaries.
But CW$_2$ results in larger $L_2$ distance, smaller SNR and PESQ for targeted attack  than for untargeted attack,
indicating that targeted attack introduces larger distortions.

Overall, targeted attack is more challenging (i.e., lower ASR and more perceptible) than untargeted attack.


% z-norm issue
% \begin{table}[]
%     \centering
%     \caption{The effectiveness and stealthiness of attacks.}
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c}
%     \hline
%       \multicolumn{2}{c|}{\multirow{2}{*}{\bf Attack}} & {\bf Effectiveness} & \multicolumn{3}{c}{\bf Stealthiness} \\ \cline{3-6}
%       \multicolumn{2}{c|}{} & {\bf ASR} & \bm{$L_2$} & {\bf SNR} & {\bf PESQ} \\ \hline
%       \multicolumn{2}{c|}{\bf FGSM} & 53.5\% & 0.537 & 28.53 & 2.23 \\ \hline
%       \multirow{6}{*}{\bf PGD} & {\bf 10} & 100\% & 0.330 & 32.77 & 2.85 \\ \cline{2-6}
%       & {\bf 20} & 100\% & 0.378 & 31.57 & 2.72 \\ \cline{2-6}
%       & {\bf 30} & 100\% & 0.385 & 31.42 & 2.70 \\ \cline{2-6}
%       & {\bf 40} & 100\% & 0.384 & 31.45 & 2.71 \\ \cline{2-6}
%       & {\bf 50} & 100\% & 0.390 & 31.31 & 2.69 \\ \cline{2-6}
%       & {\bf 100} & 100\% & 0.391 & 31.29 & 2.70 \\ \hline
%       \multicolumn{2}{c|}{\bf CW\bm{$\infty$}-30} & 100\% & 0.378 & 31.57 & 2.72 \\ \hline
%       \multirow{4}{*}{\bf CW$_2$} & {\bf 0} & 50.0\% & 0.041 & 52.99 & 4.24 \\\cline{2-6}
%       & {\bf 5} & 70.6\% & 0.058 & 49.73 & 4.10 \\ \cline{2-6}
%       & {\bf 10} & 88.5\% & 0.078 & 47.09 & 3.95\\ \cline{2-6}
%     & {\bf 20} & 100\% & 0.131 & 42.14 & 3.60 \\ \cline{2-6}
%       & {\bf 50} & 100\% & 0.476 & 30.44 & 2.46 \\ \hline
%     %   \multicolumn{2}{c|}{FAKEBOB} & 82.1\% & 0.399 & 31.06 & 2.66 \\ \hline
    % \multicolumn{2}{c|}{\bf FAKEBOB} & 80.2\% & 0.383 & 31.44 & 2.71 \\ \hline
%     \end{tabular}
%     }
%     \label{tab:evaluate-atatck}
% \end{table}


% \begin{table}[]
%     \centering \small
%     % \caption{The effectiveness and stealthiness of attacks.}
%     \caption{Effectiveness and stealthiness of targeted attacks.}
%     %\resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c}
%     \hline
%       \multicolumn{2}{c|}{\multirow{2}{*}{\bf Attack}} & \multicolumn{2}{c|}{\bf Effectiveness} & \multicolumn{3}{c}{\bf Stealthiness} \\ \cline{3-7}
%       \multicolumn{2}{c|}{} & {\bf ASR} & {\bf UTR} & \bm{$L_2$} & {\bf SNR} & {\bf PESQ} \\ \hline
%       \multicolumn{2}{c|}{\bf FGSM} & 40.2\% & 48.4\% & 0.537 & 28.53 & 2.23 \\ \hline
%       \multirow{6}{*}{\bf {PGD-$\mathbf{x}$}} & $\mathbf{x}${\bf =10} & 99.7\% & 99.7\% & 0.317 & 33.12 & 2.87 \\ \cline{2-7}
%       & $\mathbf{x}${\bf =20} & 99.7\% & 99.7\% & 0.356 & 32.10 & 2.77 \\ \cline{2-7}
%       & $\mathbf{x}${\bf =30} & 99.9\% & 99.9\% & 0.368 & 31.82 & 2.75 \\ \cline{2-7}
%       & $\mathbf{x}${\bf =40} & 99.9\% & 99.9\% & 0.373 & 31.69 & 2.74 \\ \cline{2-7}
%       & $\mathbf{x}${\bf =50} & 100\% & 100\% & 0.376 & 31.63 & 2.73 \\ \cline{2-7}
%       & $\mathbf{x}${\bf =100} & 100\% & 100\% & 0.380 & 31.53 & 2.72 \\ \hline
%       \multicolumn{2}{c|}{\bf CW\bm{$\infty$}-30} & 100\% & 100\% & 0.369 & 31.79 & 2.74 \\ \hline
%       \multirow{4}{*}{\bf CW$_2$} & $\mathbf{\kappa}${\bf =0} & 96.9\% & 97.5\% & 0.083 & 46.93 & 3.92 \\ \cline{2-7}
%       & $\mathbf{\kappa}${\bf =5} & 100\% & 100\% & 0.105 & 44.53 & 3.77 \\ \cline{2-7}
%       & $\mathbf{\kappa}${\bf =10} & 100\% & 100\% & 0.139 & 41.79 & 3.57 \\ \cline{2-7}
%     & $\mathbf{\kappa}${\bf =20} &  100\% & 100\% & 0.290 & 35.03 & 2.94 \\ \cline{2-7}
%       & $\mathbf{\kappa}${\bf =50} &  100\% & 100\% &  1.714 & 18.91 & 1.51 \\ \hline
%     \multicolumn{2}{c|}{\bf FAKEBOB} & 51.5\% & 55.4\% & 0.378 & 31.55 & 2.72 \\ \hline
%     % \multicolumn{2}{c|}{\bf FAKEBOB} &  &  &  &  \\ \hline
%     \end{tabular}
%     %}
%     \label{tab:evaluate-atatck-target}
% \end{table}


==> our-approach.tex <==
%\sen{We can not follow the previous paper structure. Before the approach and study/evaluation, we can provide an workflow picture to tell the readers what will we do in this paper. I think you can refer to my icse 2020 paper. If %you want to tone down your method.} \chengk{Answer: I have drawn an overview of study, but not sure with the suitable place to place it.}

% \section{Feature-Level Transformations}\label{sec:our-approach}
\section{Feature-Level Input Transformations}\label{sec:our-approach}
%Apart from the above input transformations,
%in this work, we propose a novel type of \emph{feature-level} transformations dedicated to SRSs, called \defensename.

%Our approach falls into the category of input transformation methods.
%We do not target model enhancement methods since they require additional training or fine-tuning, while input transformation methods can serve as a basic module for already deployed models~\cite{xie2017mitigating}.
%Besides, we do not target detection methods since it may cause false positive and degrade the user experience~\cite{TO DO}.
%In this section, we elaborate on the detail about \defensename, including main idea, implementation and  different transformation points.

\subsection{Motivation}
% \sen{Should introduce why we choose input transformation as the target instead of model enhancement and detection.}
% Our approach falls into the category of input transformation methods.
% We do not target model enhancement methods since they require additional training or fine-tuning, while input transformation methods can serve as a basic module for already deployed models~\cite{xie2017mitigating}.
% Besides, we do not target detection methods since it may cause false positive and degrade the user experience~\cite{TO DO}.
% The main idea behind \defensename \ can be understood by analysing the its difference with existing input transformation methods.
Due to the success of input transformations for mitigating adversarial images
in the image domain, input transformations also have been proposed to
mitigate adversarial voices in the speech domain. However, existing transformations for adversarial voices overlook the internal difference between image and voice recognition. Thus,
transformations are \emph{only} applied to the input waveform signals, and \emph{feature-level} transformations have never been considered before.
%
%Input transformation, such as JPEG compression~\cite{GuoRCM18} and local smoothing~\cite{Xu0Q18}, has been successfully used to mitigate adversarial images in computer vision.
%Due to promising results, some input transformations also have been used to defend against adversarial voices~\cite{das2018adagio} by pre-processing input waveform signals, such as MP3 compression~\cite{andronic2020mp3} and median smoothing~\cite{yang2018characterizing}.  However, existing transformations for adversarial voices overlook the internal differences between image and voice recognition systems. Thus,
%transformations are \emph{only} applied to the input waveform signals, and \emph{feature-level} transformations have never been considered before.


% However, most of them fail to notice the difference of image recognition and speech recognition.
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.4\textwidth]{fig/difference-exist-ours-2}
%    \caption{The major difference between input-level and feature-level transformations.}
%    \label{fig:difference-exist-ours}
%\end{figure}

For state-of-the-art neural network based image recognition, an image is directly fed to a system without feature engineering.
%In other words, feature engineering is left to be handled by the internal neurons of the network.
Due to the time-varying non-stationary property of voices, voices are not resilient enough to noises and other variations,
and waveform signals themselves cannot effectively represent speaker characteristics~\cite{voice-feature-review}.
Hence, to achieve better feature representative capacity and system performance~\cite{xiao2016speech},
SR often has an acoustic feature
extraction pipeline as shown in \figurename~\ref{fig:typical-SRSs}, which extracts acoustic features from waveforms for speaker recognition.
%SR often relies on feature engineering to extract hand-crafted features from voice waveforms (cf. \figurename~\ref{fig:typical-SRSs}) such as MFCC and PLP. %speech spectrogram~\cite{hannun2014deep}\cite{amodei2016deep}, Filter-bank~\cite{FilterBanks}\cite{li2017deep},
% based on which models trained.
When an adversarial perturbation is crafted in the waveform,
% at the inference time,
% it will also be propagated to the features during inference time.
it will also be propagated to the acoustic features.
%Finally, the adversarial example is mis-recognized by the model using the input features.

Based on the above observation, we investigate feature-level transformations to mitigate adversarial examples in SR.
%\figurename~\ref{fig:difference-exist-ours} shows the major difference between feature-level and input-level transformations.
% The research in this work
The design of our approach
is motivated by the following
questions:
(Q1) What kind of features can be transformed?
(Q2) How to transform features?
(Q3) How effective are they?
% \chengk{Question: Q3 is not mentioned in 4.2.}


%Speaker recognition models operate on these hand-crafted features rather than the raw input, unlike image recognition.
% equipped with a feature extraction module
% the model relies on hand-crafted features such as MFCC~\cite{}
% it is common practice to extract acoustic feature from speech signal for three purposes: (1) represents speaker characteristic or speech content better since the waveform is a time-varying non-stationary signal and very little information can be said from it~\cite{} (2) be more resillent to noise and other variation.


% Fig.~\ref{fig:difference-exist-ours} empathizes the major difference between \defensename \ and existing input transformation methods. Given a speech, existing methods directly pre-process the raw waveform, while \defensename \ manipulates the acoustic feature. In speech related applications, e.g., speech recognition and speaker recognition, it is common practice to extract acoustic feature from speech signal since the feature represents speaker characteristic or speech content better than the raw waveform. Various acoustic features can be utilized, including speech spectrogram~\cite{hannun2014deep}\cite{amodei2016deep}, Filter-bank~\cite{FilterBanks}\cite{li2017deep}, Mel-Frequency Cepstral Coefficients (MFCC)~\cite{muda2010voice}, and Perceptual Linear Predictive (PLP)~\cite{hermansky1990perceptual}.


\subsection{Design}\label{sec:our-approach-implementation}
%In this section, we present our solution addressing Q1 and Q2, while Q3 is studied in
%Section~\ref{sec:evaluation}.

To address Q1, we have to understand what kind of features are used in SR.
\figurename~\ref{fig:different-features} shows a typical flow of feature processing in SR.
% First, the \emph{original features} (e.g., MFCC or PLP) are extracted from an input raw waveform. %speech spectrogram~\cite{amodei2016deep}, Filter-bank~\cite{FilterBanks},
First, the \emph{original features} (e.g., MFCC or Filter-Bank) are extracted from an input raw waveform. %speech spectrogram~\cite{amodei2016deep}, Filter-bank~\cite{FilterBanks},
Next, to capture temporal information, time-derivative features including first-order and/or second-order time derivatives~\cite{xiao2016speech}
are % iteratively
successively
extracted from and added into the original features, leading to the \emph{delta features}.
After that, cepstral mean and variance normalization
% (CMVN)~\cite{viikki1998cepstral}
(CMVN)~\cite{speech-processing-book}
is applied to the delta features
which reduces channel and reverberation effects, resulting in \emph{cmvn features}.
Finally, voice activity detection (VAD)~\cite{sohn1999statistical} is utilized to remove the unvoiced frames from the cmvn features and obtain the \emph{final features}.
Therefore, these four types of features could be transformed, which may disrupt adversarial perturbations at the feature level.
% Note that \figurename~\ref{fig:different-features} only depicts a typical feature processing flow and there may be some exceptions, e.g., using cepstral mean normalization (CMN)~\cite{speech-processing-book} instead of CMVN.

To address Q2, a straightforward idea is to directly extend the existing transformations from input waveforms to features.
However, such extension is \emph{not} trivial due to the following reasons.
(1) All the transformations mentioned in Section~\ref{sec:input-transformation} work on voice waveforms, each of which
is a vector, where the value at each index denotes the magnitude at the corresponding sample point.
While features of an input voice
% at each step
are represented by a matrix,
one row of features per frame.
% This difference prevents from frequency-related transformations (i.e., DS, LPF, BPF) and speech compression.
This difference prevents frequency domain transformations (i.e., DS, LPF, and BPF) and speech compressions from being extended to the feature level.
(2) The mapping from waveforms to features is not linear,
and a small perturbation in the input voice may result in a large
perturbation at the feature level.
% This difference prevents from QT, AT, AS and MS transformations
This difference refuses time domain transformations (i.e., QT, AT, AS, and MS)
which assumed that perturbations are small and/or sensitive to noises.


Inspired by speech compressions, we propose \defensename (\defensenameabbr), a feature compression approach
to disrupt perturbations at the feature level. For a feature matrix $\mathcal{M}$ with $N$ frames
and each frame consists of $d$ features, we regard the matrix $\mathcal{M}$ as $N$ data points in $d$-dimensional space and
partition $N$ data points into $K$ clusters for a given parameter $K<N$.
Then, all data points in one cluster are represented by a representative vector.
Finally, $K$ representative vectors are combined to form the new feature matrix $\mathcal{M}'$.
We denote the ratio between $N$ and $K$ by $cl_r=\frac{K}{N}$.


To partition $N$ data points into $K$ clusters, various clustering methods such as kmeans~\cite{hartigan1979algorithm}, soft-kmeans~\cite{mackay2003information}, and Gaussian Mixture Model~\cite{fraley1998many}
could be leveraged. In this work, we use kmeans and its variant warped-kmeans~\cite{LeivaV13}
and leave others as future work.
Compared to kmeans, warped-kmeans preserves the temporal dependency of the data by imposing some constraints on the partition operation,
thus is more suitable to cluster sequential data.
% \chengk{We highlight that kmeans-based \defensenameabbr utilizes the property
% that text-independent SRSs does not rely on temporal dependency
% % since it does not maintain the order of feature vectors sequence.
% since it may shuffle the timing order of feature vectors sequence.
% }
For both kmeans and warped-kmeans, the representative vector of a cluster is the average of all data points within this cluster
(cf. Appendix~\ref{sec:FeCo-appendix} for more details).
% \chengk{(Question: I don't think so, suggest deleting this sentence) which
%can be seen as a combination of MS and BPF transformations at feature level.}
% \chengk{We implemented our approach \defensenameabbr in Pytorch~\cite{} library which supports auto-auto-differentiation, making \defensenameabbr totally differentiable.}
% Furthermore, both kmeans and warped-kmeans are randomized methods, thus our approach is randomized.


Our approach could be applied to any types of features mentioned above, i.e., original, delta, cmvn, and final features.
% In the rest of this paper, we use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), \defensename-final (\defensenameabbr-f) to mark which feature \defensename \ transforms.
We use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), and \defensename-final (\defensenameabbr-f) to denote
these four concrete feature-level transformations, which are randomized and differentiable (cf. Appendix~\ref{sec:FeCo-appendix}).
We will thoroughly evaluate their effectiveness (i.e., Q3) later.
%Both kmeans and warped-kmeans are randomized methods, thus our approach is randomized.
%\chengk{Furthermore, we implemented \defensenameabbr in Pytorch~\cite{PaszkeGMLBCKLGA19} library
%which supports auto-differentiation, making \defensenameabbr totally differentiable.}


%
%
%Hence, one of the adjustable parameters of \defensename \ is the clustering method, denoted as $cl_m$.
%In this work, we adopt kmeans and one of its variant warped-kmeans~\cite{LeivaV13}. We leave the discussion of other cluster methods as our future work.
%Compared to kmeans, warped-kmeans preserves the temporal dependency of the data by imposing some constraints on the partition operation, thus is more suitable to cluster sequential data.
%For both kmeans and warped-kmeans, the representative vector of a cluster is the average of all data points within this cluster.
%Since kmeans and warped-kmeans randomly initialize $K$ clusters, our approach \defensename\ introduces randomized effect, as shown in the last column in \tablename~\ref{tab:input-transform}.
%Another adjustable parameter of \defensename \ , denoted by $cl_r$, is the ratio between $N$ and $K$, i.e., $cl_r=\frac{K}{N}$.
% parameter



%
%What is more, it is usually beneficial to further process the original feature (e.g., MFCC, PLP) to achieve better feature representative capacity and system performance~\cite{xiao2016speech}. Fig.~\ref{fig:different-features} displays a typical process flow. Firstly, to capture temporal information, we concatenate the original feature with time-derivative feature~\cite{xiao2016speech}, including delta feature (first-order time derivative)~\cite{xiao2016speech} and acceleration feature (second-order time derivative)~\cite{xiao2016speech}. Call it delta feature after this step. Next, we apply Cepstral Mean and Variance Normalization (CMVN)~\cite{viikki1998cepstral} to delta feature to reduce channel and reverberation effects, resulting in cmvn feature. Finally, we utilize Voice Activity Detection (VAD)~\cite{sohn1999statistical} to remove the unvoiced frames of cmvn feature and obtain the final feature.
%
%When adversarial perturbation is crafted in the waveform, the perturbation will also be propagated to the feature.
%Since the feature is the direct input to the models and is more co-related with models' output than the raw waveform, we propose to apply input transformation on the feature level with the attempt to disrupt the perturbation in the feature.
%Figure.~\ref{fig:difference-exist-ours} empathizes the major difference between \defensename \ and existing input transformation methods. Given a speech, existing methods directly pre-process the raw waveform, while \defensename \ manipulates the acoustic feature.

%To eliminate the adversarial perturbation from the feature, we propose \defensename, a feature compression approach.

%Specifically, suppose the feature matrix $M$ has the dimension of $N\times d$ which means the corresponding speech is framed into $N$ frames and each frame is represented by a $d$ dimension vector.
%\defensename \ treats $M$ as $N$ data points and partitions them into $K$ clusters ($K<N$). Then all data points in one cluster are represented by a representative vector of this cluster. Finally $K$ representative vectors are %combined to form a new feature matrix. The representative vector varies with the implementation of \defensename \ (cf. section \ref{sec:our-approach-implementation}).

% {\defensename \ is a process of feature compression, i.e., from $N$ frames to $K$ frames, during which the adversarial perturbation is disrupted. Hence, \defensename \ can be used to defend adversarial examples.}
%{\defensename\ compresses the feature from $N$ frames to $K$ frames, during which the adversarial perturbation is disrupted. Hence, \defensename \ can be utilized to defend adversarial examples.}
% difference waveform --> feature
% how it works ?
% why it works ?

%To divide $N$ frames into $K$ clusters, \defensename \ utilizes clustering algorithms. There are various clustering methods, such as kmeans~\cite{hartigan1979algorithm}, soft-kmeans~\cite{mackay2003information}, Gaussian Mixture Model (GMM)~\cite{fraley1998many}, etc. Hence, one of the adjustable parameters of \defensename \ is the clustering method, denoted as $cl_m$.
%In this work, we adopt kmeans and one of its variant warped-kmeans~\cite{LeivaV13}. We leave the discussion of other cluster methods as our future work.
%Compared to kmeans, warped-kmeans preserves the temporal dependency of the data by imposing some constraints on the partition operation, thus is more suitable to cluster sequential data.
%For both kmeans and warped-kmeans, the representative vector of a cluster is the average of all data points within this cluster.
%Since kmeans and warped-kmeans randomly initialize $K$ clusters, our approach \defensename\ introduces randomized effect, as shown in the last column in \tablename~\ref{tab:input-transform}.
%Another adjustable parameter of \defensename \ , denoted by $cl_r$, is the ratio between $N$ and $K$, i.e., $cl_r=\frac{K}{N}$.
%% parameter
%% representative vector kmeans: L2
%% different tasks, different algo. text-dependent speaker recognition / speech recognition, should use algo that keeps time dependency.
%
%In addition, our approach \defensename \ has the choice to transform any of the four features in \figurename~\ref{fig:different-features}, i.e., original, delta, cmvn and final features.
%% In the rest of this paper, we use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), \defensename-final (\defensenameabbr-f) to mark which feature \defensename \ transforms.
%We use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), \defensename-final (\defensenameabbr-f) to mark which feature \defensename \ transforms.

% \subsection{Transforming Different Features}
% % As shown in Fig.~\ref{fig:different-features}, to further improve the representative capacity of the feature, we usually append static feature\footnote{Static feature is the original feature, such as MFCC, PLP, and etc.} with dynamic feature (i.e., delta and acceleration features), Cepstral Mean Normalization (CMN) or Cepstral Mean and Variance Normalization (CMVN), and finally apply Voice Activity Detection (VAD) to remove unvoiced frames.
% In speech related application, it is usually beneficial to process the original feature (e.g., MFCC, PLP) to achieve better feature representative capacity and system performance~\cite{xiao2016speech}. Fig.~\ref{fig:different-features} displays a typical process flow. Firstly, to capture temporal information, we concatenate the original feature with time-derivative feature~\cite{xiao2016speech}, including delta feature (first-order time derivative)~\cite{xiao2016speech} and acceleration feature (second-order time derivative)~\cite{xiao2016speech}. Call it delta feature after this step. Next, we apply Cepstral Mean and Variance Normalization (CMVN)~\cite{viikki1998cepstral} to delta feature to reduce channel and reverberation effects, resulting in cmvn feature. Finally, we utilize Voice Activity Detection (VAD)~\cite{sohn1999statistical} to remove the unvoiced frames of cmvn feature and obtain the final feature.

% Hence, herein \defensename \ has the choice to transform any of the four features, i.e., original, delta, cmvn and final features.
% % In the rest of this paper, we use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), \defensename-final (\defensenameabbr-f) to mark which feature \defensename \ transforms.
% We use \defensename-origin (\defensenameabbr-o), \defensename-delta (\defensenameabbr-d), \defensename-cmvn (\defensenameabbr-c), \defensename-final (\defensenameabbr-f) to mark which feature \defensename \ transforms.



==> system-desgin-implement.tex <==

% \section{System Design and Implementation}
\section{\platformname Platform}\label{sec:design-implement}
%\sen{Shall we highlight the purpose that we propose such a platform?}
% modules: model / dataset / attack / defense / attack metric / defense metric / BPDA and EOT wrapper
To advance future research on adversarial examples in SR,
in this section, we present the design and implementation of a SECurity analysis platform for SR, named \platformname~\cite{SEC4SR}.
Our platform is designed to be modular, flexible and extensible
% and implemented using Pytorch~\cite{}, a popular framework for deep learning research,
so that new models, datasets,
attacks and defenses can be easily integrated into the platform to comprehensively and systematically evaluate
their performance.



% \subsection{Modular Design}


The overview of our platform is shown in \figurename~\ref{fig:overview-platform}, consisting of
the following five main components.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/overview-platform-3}\vspace*{-3mm}
    \caption{Overview of our platform \platformname.}
    \label{fig:overview-platform}\vspace*{-3mm}
\end{figure}

%In pursuit of readability, comprehensibility, easy-of-use and extendability, \platformname \ takes fully-modular design and consists of five components, as shown in Fig.~\ref{fig:overview-platform}.

\smallskip
% \noindent {\bf Model Component (MC).}
% In speaker recognition domain, researchers evaluated on different models the capacity of their attacks or the model resilience improvement brought by their defenses. These models vary with each other in front-end features (MFCC or PLP), model types (traditional model or neural network), model architectures (xvector~\cite{snyder2018x}, AudioNet~\cite{becker2018interpreting} or ResNet~\cite{he2016deep}), training algorithms (unsupervised or supervised), back-end scoring methods (COSS or PLDA), training sets (VoxCeleb~\cite{nagrani2017voxceleb} or Librispeech~\cite{panayotov2015librispeech}) and so on. Different benchmarks make their results hard to compare with each other. Hence, the core function of MC is providing several standard models on which future researchers are encouraged to benchmark on.

% \smallskip\noindent {\bf Dataset Component (DAC).}
% In the filed of adversarial image classification, MNIST, CIFAR, CIFAR-10 and ImageNet are commonly-used datasets, which is beneficial for fair comparison of the results.
% However, the usage of datasets in the research of adversarial speaker recognition is rather diverse.
% Researchers use different public speech datasets or maybe randomly choose a subset of voices for experiments.
% In addition, since most prior works only take into account CSI-NE task, the datasets for CSI-E, SV and OSI remain unfixed.
% DAC supplies several standard datasets to deal with this problem.

% \noindent {\bf Model Component (MC) \& Dataset Component (DAC).}
% Over the past few years, adversarial speaker recognition has attracted increasing attention with number of works either uncovering the security implication of SR under attacks~\cite{chen2019real}\cite{li2020adversarial}\cite{xie2021real}\cite{abs-1801-03339} or defending SR systems against such security threat~\cite{jati2021adversarial}.
% However, previous works benchmark their attack and defense algorithms on different models and datasets.
% These models vary with each other in front-end features, model architectures, training algorithms, model parameters, back-end scoring methods and so on.
% % Regarding the datasets, different free public or even charged-access speech datasets are adopted,
% Regarding the datasets, different free public speech datasets are adopted,
% and sometimes for ease of experiment, a subset of voices are \textit{randomly} chosen from these datasets.
% In addition, to study CSI-E, SV and OSI tasks, we need three specific datasets which contain enrollment voices, enrolled speakers' voices and impostors' voices respectively (cf. \tablename~\ref{tab:DAC}).
% Since most prior works only take into account CSI-NE, the splitting of these three datasets has not been standarly set up.
% The lack of a standard benchmark regarding both models and datasets makes it challenging to compare the efficacy of proposed methods with each other.
% To tackle this problem, we provide three speaker recognition models in MC, covering typical and state-of-the-art architectures, and five datasets in ADC, covering different SR tasks.
% We strongly encourage future researchers to benchmark on these models and datasets to fully gauge the quality of their proposed methods.
% We hope the benchmark can help researcher better improve their methods, thus accelerate the growth of adversarial speaker recognition.

\smallskip\noindent {\bf Model component (MC).}
Adversarial attacks and defenses in SR have attracted increasing attentions~\cite{chen2019real,du2020sirenattack,ASGBWYST19,li2020adversarial,abs-1801-03339,jati2021adversarial,AWBPT20}.
However, previous works benchmark their attacks and defenses on different SRSs,
varying in front-end features (e.g., MFCC and PLP), model architectures, recognition tasks, training algorithms, % (e.g., unsupervised and supervised),
and back-end scoring methods.
This hampers researchers to comprehensively and systematically evaluate the proposed methods.


To tackle this problem, \platformname provides 3 mainstream SRSs including
ivector-PLDA~\cite{kaldi-ivector-plda} and xvector-PLDA~\cite{kaldi-xvector-plda} that are pre-trained models of the popular open-source platform KALDI having 10k stars and 4.4k forks on GitHub~\cite{kaldi},
and a one-dimension convolution neural network based model AudioNet that was proposed in \cite{becker2018interpreting} and studied in \cite{jati2021adversarial}.
These models cover all the recognition tasks.
Details of these models are summarized in \tablename~\ref{tab:MC}.



%Over the past few years, adversarial speaker recognition has attracted increasing attention with number of works either uncovering the security implication of SR under attacks~\cite{chen2019real}\cite{li2020adversarial}\cite{xie2021real}\cite{abs-1801-03339} or defending SR systems against such security threat~\cite{jati2021adversarial}.
%However, previous works benchmark their attack and defense algorithms on different speaker recognition models.
%These models vary with each other in front-end features, model architectures, training algorithms, model parameters, back-end scoring methods and so on.
%The lack of a standard benchmark regarding models makes it challenging to compare the efficacy of proposed methods with each other.
%To tackle this problem, we provide three speaker recognition models in MC, covering typical and state-of-the-art architectures, including ivector-PLDA, xvector-PLDA and AudioNet. Difference of their embedding type, front-end features, training algorithms and back-end scoring methods between them are highlighted in \tablename~\ref{tab:MC}.
% Specifically, we use the pre-trained ivector-PLDA model~\cite{kaldi-ivector-plda} released by the popular open-source platform KALDI, having 10k stars and 4.4k forks on github~\cite{kaldi}.
% \chengk{TO DO: about xvector-PLDA.}
% We use AudioNet~\cite{becker2018interpreting}, a one-dimension Convolution Neural Network (CNN) based model.

%Specifically, both ivector-PLDA~\cite{kaldi-ivector-plda} and xvector-PLDA~\cite{kaldi-xvector-plda} are pre-trained models released by popular open-source platform KALDI, having 10k stars and 4.4k forks on github~\cite{kaldi}.
%AudioNet, a one-dimension Convolution Neural Network (CNN) based model, is proposed in \cite{becker2018interpreting} and studied in \cite{jati2021adversarial}.

\smallskip\noindent {\bf Dataset component (DAC).}
Open-access voice datasets are provided for training and testing of speaker or speech recognition,
but not for evaluating adversarial attacks and defenses.
The latter often requires different types of voice sets for different recognition tasks.
For instance, enrollment speakers are not required for the CSI-NE task, but are required for the other tasks (e.g., CSI-E, SV, and OSI).
Imposters are not required for the CSI-E and CSI-NE tasks, but are required for the SV and OSI tasks.
% Since there is no uniform set up of voice sets for each recognition task when evaluating adversarial attacks or defenses,
% previous studies \textit{randomly} choose different subsets of voices from different voice datasets
% for the same recognition task~\cite{chen2019real}\cite{foolhd}\cite{WangGX20}\cite{LiZXZ0M020}.
{Since there is no uniform set up of voice sets for evaluating adversarial attacks or defenses,
previous studies \textit{randomly} choose different subsets of voices from different voice datasets~\cite{chen2019real, shamsabadi2021foolhd, WangGX20, LiZXZ0M020}.}
This hinders comprehensive and systematic evaluation of adversarial attacks and defenses.


To solve this problem, \platformname provides 5 datasets: Spk$_{10}$-enroll, Spk$_{10}$-test, Spk$_{10}$-imposter, Spk$_{251}$-train, and Spk$_{251}$-test,
covering the required datasets for all the recognition tasks (i.e., CSI-NE, CSI-E, SV, and OSI).
The datasets are summarized in \tablename~\ref{tab:DAC}.

% Regarding the datasets, different free public or even charged-access speech datasets are adopted,
%Regarding the datasets, previous works adopt different free public speech datasets, and sometimes for ease of experiment, a subset of voices are \textit{randomly} chosen from these datasets.
%In addition, to study CSI-E, SV and OSI tasks, we need three specific datasets which contain enrollment voices, enrolled speakers' voices and impostors' voices respectively (cf. \tablename~\ref{tab:DAC}).
%Since most prior works only take into account CSI-NE, the splitting of these three datasets has not been standarly set up.
%The lack of a standard benchmark regarding datasets make it more difficult to conduct fair result comparison.
%To solve this problem, we provide five datasets in ADC, covering different SR tasks, namely, Spk$_{10}$-enroll, Spk$_{10}$-test, Spk$_{10}$-imposter, Spk$_{251}$-train and Spk$_{251}$-test, the detail of which is depicted in \tablename~\ref{tab:DAC}.

% Spk$_{10}$-enroll and Spk$_{10}$-test are created for CSI-E task.
Spk$_{10}$-enroll consists of 10 speakers (5 males and 5 females), 10 voices per speaker.
The speakers are randomly selected from the ``test-other'' and ``dev-other'' subsets of the popular dataset Librispeech~\cite{panayotov2015librispeech,LiZJXZWM020,zhang2021attack,jati2021adversarial,chen2019real}.
For each speaker, we select the top-10 longest voices in order to have better enrollment embedding~\cite{ParkYKKA17, app9183697}. The voices in Spk$_{10}$-enroll are used for speaker enrollment
of the CSI-E, SV, and OSI tasks.
%
% Spk$_{10}$-test (resp. Spk$_{10}$-imposter) consists  10 speakers (5 males and 5 females), 100 voices per speaker.
% Spk$_{10}$-test has the same speakers as Spk$_{10}$-enroll, but the voices of each speaker
% are the top-10 longest voices in the remaining ones.
% Spk$_{10}$-imposter has distinct speakers from the ``dev-other" subset of Librispeech
% and their voices are the top-10 longest voices.
Spk$_{10}$-test (resp. Spk$_{10}$-imposter) consists 10 speakers (5 males and 5 females), 100 randomly selected voices per speaker.
Spk$_{10}$-test has the same speakers as Spk$_{10}$-enroll, but distinct voices.
The speakers in Spk$_{10}$-imposter are randomly chosen from the ``train-other-500" subset of Librispeech, but are different from the speakers in Spk$_{10}$-test.
Both Spk$_{10}$-test and Spk$_{10}$-imposter can be used for adversarial attacks on the CSI-E, SV, and OSI tasks,
where the speakers of Spk$_{10}$-test have been enrolled, but
the speakers of Spk$_{10}$-imposter have not been enrolled.



%Then their top ten longest-duration voices are pickled out to form Spk$_{10}$-enroll, which is used as enrollment voices during enrollment phrase. Excluding the enrollment voices, we randomly select 100 voices for each speaker, resulting in 1000 voices totally in Spk$_{10}$-test, which are used to generate adversarial examples. Note that we do not provide training dataset for CSI-E task for two reasons: (1) Ivector-PLDA and xvector-PLDA in MC are per-trained models, thus require no training. (2) For CSI-E task, it is not necessarily that enrolled speakers are among training speakers, thus one can utilize arbitrary training sets, such as Spk$_{251}$-train.
%After excluding the speakers in Spk$_{10}$-enroll and Spk$_{10}$-test, we randomly select another 10 speakers (5 male, 5 female) from Librispeech and randomly select 100 voices for each speaker, composing Spk$_{10}$-imposter. For SV and OSI task, we are more interested in whether a voice uttered by a source speaker out of the enrolled speakers group can be misclassified by one of the enrolled speakers, so it is recommended that Spk$_{10}$-imposter is used to generate adversarial examples in SV and OSI tasks.

Both Spk$_{251}$-train and Spk$_{251}$-test
are taken from the ``train-clean-100'' subset of Librispeech,
each of which has the same 251 speakers (126 males and 125 females).
Following \cite{jati2021adversarial}, for each speaker, 90\% of his/her voices are added into Spk$_{251}$-train,
and the remaining 10\% are added into Spk$_{251}$-test.
Spk$_{251}$-train can be used to train background
models while Spk$_{251}$-test can be used for adversarial attacks
on the CSI-NE task.
Since there are no overlapping speakers among Spk$_{251}$-train, Spk$_{10}$-test, and Spk$_{10}$-imposter,
if one prefers to attack the CSI-NE task using the voices
of the speakers that are not in Spk$_{251}$-train,
voices in Spk$_{10}$-enroll, Spk$_{10}$-test and Spk$_{10}$-imposter could be used.
%
%
%Spk$_{251}$-train and Spk$_{251}$-test are from ``train-clean-100" subset of Librispeech~\cite{panayotov2015librispeech}, which contains 251 speakers. Following \cite{jati2021adversarial}, for each speaker, 90\% of the utterances are selected as training set, and the remaining 10\% as test set, composing Spk$_{251}$-train and Spk$_{251}$-test respectively. Spk$_{251}$-train and Spk$_{251}$-test are suitable for CSI-NE task since the set of speakers to be identified includes exactly all training speakers.
% \chengk{TO DO: Dataset for SV and OSI tasks.}

\begin{table}[t]
    \centering
     \caption{Models in MC, where T/D denote traditional/deep model, US/S stand for unsupervised/supervised learning.}
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{c|c|c|c}
    \hline
     & {\bf ivector-PLDA} & {\bf xvector-PLDA} & {\bf AudioNet} \\ \hline
      \begin{tabular}[c]{@{}c@{}}{\bf Embedding type}\end{tabular} & T & D & D \\ \hline
      {\bf Feature type} & MFCC & MFCC & MFCC \\ \hline
      {\bf Add delta} & \cmark & \xmark & \xmark \\ \hline
      {\bf Add acceleration} & \xmark & \cmark & \xmark \\ \hline
      {\bf Apply CMVN} & \cmark & \cmark & \xmark \\ \hline
      {\bf Apply VAD} & \cmark & \cmark & \xmark \\ \hline
      {\bf \#Feature dim} & 72 & 30 & 32 \\ \hline
      {\bf Training algorithm} & US & S & S \\ \hline
      {\bf Scoring method} & PLDA & PLDA & COSS \\ \hline
    \end{tabular}
    }
    \label{tab:MC} \vspace*{-2mm}
\end{table}
\begin{table}[t]
    \centering
\setlength\tabcolsep{2pt}
    \caption{Voice datasets in DAC, where x-y(z) indicates that the minimal, maximal and average length of voices are x, y, z.}
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \hline
         & {\bf Spk$_{10}$-enroll} & {\bf Spk$_{10}$-test} & {\bf Spk$_{10}$-imposter} & {\bf Spk$_{251}$-train} & {\bf Spk$_{251}$-test} \\ \hline
         {\bf Task} & \multicolumn{3}{c|}{CSI-E/SV/OSI } & \multicolumn{2}{c}{CSI-NE} \\ \hline  %& CSI-E & SV/OSI
      %   {\bf Source} & Librispeech & Librispeech & Librispeech &  Librispeech & Librispeech \\ \hline
         {\bf \#Speakers} & 10(5M,5F) & 10(5M,5F) & 10(5M,5F) &
        %  {\begin{tabular}[c]{@{}c@{}} 251\\(12757M,12895F)\end{tabular}}
        {\begin{tabular}[c]{@{}c@{}} 251\\(126M,125F)\end{tabular}}
         &
        %  {\begin{tabular}[c]{@{}c@{}} 251\\(1440M,1447F)\end{tabular}}
        {\begin{tabular}[c]{@{}c@{}} 251\\(126M,125F)\end{tabular}}
         \\ \hline
         {\bf \#Voices} & 10$\times$10 & 100$\times$10 & 100$\times$10 & 25652 & 2887 \\ \hline
         {\bf Length} & 3--21s (7.2s) & 1--15s(4.3s) & 1--17s(8.33s) & 1--24s (12.3s) & 1--19s (11.7s) \\ \hline
    \end{tabular}
    }
    \label{tab:DAC} \vspace*{-2mm}
\end{table}

\smallskip\noindent {\bf Attack Component (AC).}
The main function of AC is to explore vulnerabilities of SRSs by launching adversarial attacks.
AC implements the representative and state-of-the-art attacks mentioned in Section~\ref{sec:review-attacks},
namely, 4 white-box attacks: FGSM, PGD and CW$_{\bm{\infty}}$, CW$_2$; and 2 black-box attacks: FAKEBOB and SirenAttack.
Note that CW$_{\bm{\infty}}$ is implemented by adopting the loss function of CW  but optimizing by PGD, the same as \cite{madry2017towards} and \cite{dong2020adversarial},
in order to improve the attack efficiency.

\smallskip\noindent {\bf Defense Component (DEC).}
The main function of DEC is to protect SRSs and improve their resistance to adversarial examples.
DEC implements all defense methods mentioned in Section~\ref{sec:review-defenses}
and Section~\ref{sec:our-approach}, including robust training and input-/feature-level transformations.
Specifically, for robust training, we implement both FGSM and PGD based adversarial training.
For input transformation, we implement 14 input transformations and 8 novel feature transformations.

\smallskip\noindent {\bf Adaptive Attack Component (ADAC).}
ADAC is mainly used to implement adaptive attacks when the adversary aims to circumvent a chosen defense.
Currently, ADAC includes both BPDA, EOT and NES (cf. Section~\ref{sec:adaptive-attack-2-defense}).
They are implemented as standalone wrappers so that they can be easily plugged into attacks
to mount adaptive attacks. %Currently this component implements two adaptive attack techniques, i.e., BPDA and EOT .
% In ADAC, we implement BPDA and EOT as two standalone modules such that they can be easily plugged into basic attacks in AC to launch adaptive attacks.

We strongly encourage researchers to
add new models, datasets, attacks and defenses into our platform,
and  comprehensively and
systematically evaluate them using our platform.
We expect our platform can advance future research on adversarial examples in SR.


% \subsection{Implementation}
% In MC, we provide three models, including ivector-PLDA, xvector-PLDA and AudioNet. Difference of embedding type, front-end features, training algorithms and back-end scoring methods between them are highlighted in \tablename~\ref{tab:MC}.
% % Specifically, we use the pre-trained ivector-PLDA model~\cite{kaldi-ivector-plda} released by the popular open-source platform KALDI, having 10k stars and 4.4k forks on github~\cite{kaldi}.
% % \chengk{TO DO: about xvector-PLDA.}
% % We use AudioNet~\cite{becker2018interpreting}, a one-dimension Convolution Neural Network (CNN) based model.
% Specifically, both ivector-PLDA~\cite{kaldi-ivector-plda} and xvector-PLDA~\cite{kaldi-xvector-plda} are pre-trained models released by popular open-source platform KALDI, having 10k stars and 4.4k forks on github~\cite{kaldi}.
% AudioNet, a one-dimension Convolution Neural Network (CNN) based model, is proposed in \cite{becker2018interpreting} and studied in \cite{jati2021adversarial}.

% In DAC, we supply four datasets, namely, Spk$_{10}$-enroll, Spk$_{10}$-test, Spk$_{251}$-train and Spk$_{251}$-test, the detail of which is depicted in \tablename~\ref{tab:DAC}.
% In DAC, we supply five datasets, namely, Spk$_{10}$-enroll, Spk$_{10}$-test, Spk$_{10}$-imposter, Spk$_{251}$-train and Spk$_{251}$-test, the detail of which is depicted in \tablename~\ref{tab:DAC}.

% % Spk$_{10}$-enroll and Spk$_{10}$-test are created for CSI-E task.
% Spk$_{10}$-enroll is used to enroll speakers, and Spk$_{10}$-test (resp. Spk$_{10}$-imposter), is created for CSI-E task (resp. SV and OSI tasks).
% We first randomly select ten speakers (5 female, 5 male) from Librispeech~\cite{panayotov2015librispeech} dataset. Then their top ten longest-duration voices are pickled out to form Spk$_{10}$-enroll, which is used as enrollment voices during enrollment phrase. Excluding the enrollment voices, we randomly select 100 voices for each speaker, resulting in 1000 voices totally in Spk$_{10}$-test, which are used to generate adversarial examples. Note that we do not provide training dataset for CSI-E task for two reasons: (1) Ivector-PLDA and xvector-PLDA in MC are per-trained models, thus require no training. (2) For CSI-E task, it is not necessarily that enrolled speakers are among training speakers, thus one can utilize arbitrary training sets, such as Spk$_{251}$-train.
% After excluding the speakers in Spk$_{10}$-enroll and Spk$_{10}$-test, we randomly select another 10 speakers (5 male, 5 female) from Librispeech and randomly select 100 voices for each speaker. For SV and OSI task, we are more interested in whether a voice uttered by a source speaker out of the enrolled speakers group can be misclassified by one of the enrolled speakers, so it is recommended that Spk$_{10}$-imposter is used to generate adversarial examples in SV and OSI tasks.

% Spk$_{251}$-train and Spk$_{251}$-test are from ``train-clean-100" subset of Librispeech~\cite{panayotov2015librispeech}, which contains 251 speakers. Following \cite{jati2021adversarial}, for each speaker, 90\% of the utterances are selected as training set, and the remaining 10\% as test set, composing Spk$_{251}$-train and Spk$_{251}$-test respectively. Spk$_{251}$-train and Spk$_{251}$-test are suitable for CSI-NE task since the set of speakers to be identified includes exactly all training speakers.
% % \chengk{TO DO: Dataset for SV and OSI tasks.}

% In AC, we implement five attacks as we mentioned in section~\ref{sec:review-attacks}. Specifically, the implemented attacks cover three white-box attacks: FGSM, PGD and CW$_{\bm{\infty}}$, CW$_2$; and one black-box attacks: FAKEBOB. Note that CW$_{\bm{\infty}}$ is implemented by adopting the CW loss but optimizing by PGD, the same as \cite{madry2017towards} and \cite{dong2020adversarial}.

% In DEC, we currently implement two categories of defenses:  adversarial training and input transformation. For adversarial training, we implement FGSM and PGD adversarial training. For input transformation, we implement 15 defenses, including 14 existing methods listed in section \ref{sec:review-defenses} and our proposed method \defensename.

% In ADAC, we implement BPDA and EOT as two standalone modules such that they can be easily plugged into basic attacks in AC to launch adaptive attacks.




% \begin{table}[]
%     \centering
%     \caption{Detail of datasets in DAC.}
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c}
%     \hline
%          & {\bf Spk$_{10}$-enroll} & {\bf Spk$_{10}$-test} & {\bf Spk$_{251}$-train} & {\bf Spk$_{251}$-test} \\ \hline
%          {\bf Task} & CSI-E & CSI-E & CSI-NE & CSI-NE \\ \hline
%          {\bf Source} & Librispeech & Librispeech & Librispeech & Librispeech \\ \hline
%          {\bf \#Speakers} & 10(5M,5F) & 10(5M,5F) & 251(12757M,12895F) & 251(1440M,1447F) \\ \hline
%          {\bf \#Voices} & 100 & 1000 & 25652 & 2887 \\ \hline
%          {\bf duration} & 3-21s (7.2s) & 1-15s(4.3s) & 1-24s (12.3s) & 1-19s (11.7s) \\ \hline
%     \end{tabular}
%     }
%     \label{tab:DAC}
% \end{table}


==> threat-model.tex <==
% \subsection{Threat Model and Assumptions}
% \subsection{Threat Model}
\section{Threat Model}
In this section, we define the threat model, including adversary's goals, capabilities, and obtained knowledge.
% following the recommendation for describing threat model in \cite{evaluate-robustness}.

% A SR model can be denoted as ${\tt SR}_{\text{task}}(x):\mathcal{X} \rightarrow \mathcal{Y}$, where
% % $x\in\mathcal{X}\subset \mathbb{R}^d$
% $x\in\mathcal{X}$
% is the input voice, and $\mathcal{Y}$ the
% % space of decision.
% decision space.
% For CSI task, $\mathcal{Y}=\{1,2,\cdots,K\}$ with $K (K>1)$ being the number of candidate speakers. For SV task, $\mathcal{Y}=\{{\tt accept}, {\tt reject}\}$. For OSI task, $\mathcal{Y}=\{1,2,\cdots,K,{\tt reject}\}$.

% \subsubsection{Adversary's Goals}
% \subsection{Adversary's Goals}
\smallskip\noindent {\bf Adversary's goal.}
% Based on the recognition task, the ground-truth of the benign voice and untargeted/targeted attack, an adversary can achieve different goals of crafting adversarial examples.
An adversary can achieve different goals of crafting adversarial examples by using benign voices with different ground-truths and launching untargeted/targeted attacks on different recognition tasks.
% In this work, we study untargeted attack on CSI task, that is, given an benign voice with ground-truth $y\in\{1,2,\cdots,M\}$, the adversary aims to cause misclassification to the SR model (i.e., ${\tt SR}_{\text{CSI}}(x^{adv})\neq y$).
In this work, we focus on the goal of causing untargeted misclassification to the CSI system,
% that is, given a benign voice $x$ with ground-truth $y\in\{1,2,\cdots,M\}$,
% crafting an adversarial voice $x^{adv}$ such that ${D}_{\text{CSI}}(x^{adv})\neq y$.
that is, given a benign voice $x$ uttered by a speaker in the group,
crafting an adversarial voice $x^{adv}$ such that the system recognizes $x^{adv}$ as from another speaker within the group.
% ${\tt SR}_{\text{CSI}}(x^{adv})\neq y$.
% This corresponds to two attack scenarios in the real life.
% The first one: the adversary is a criminal and he is one of the speakers in the SR model (e.g., criminal detection network), and he manipulates his voices such that they are recognized as another speaker to bypass the detection.
% The second one: the adversary manipulates the voices of an enrolled speaker such that these voices are wrongly recognized, causing Denial-of-service to this speaker.
We highlight two practically feasible attack scenarios associated with this goal:
1) the adversary crafts adversarial voices for the super user of smart home who has exclusive control over some devices. These voices are wrongly recognized as arbitrary ordinary users, causing Denial-of-Service (DoS) to the super user;
2) the criminal manipulates his voices to fool the voiceprint-based criminal detection system to recognize him as arbitrary legitimate citizens.
% \chengk{TO DO: attack scenario in real life. crime/Dos}
% In addition to misclassification, the adversary attempts to make $x^{adv}$ still sounds like speaker $y$ from the perspective of human beings.

% \subsubsection{Adversary's Capabilities}
% \subsection{Adversary's Capabilities}
\smallskip\noindent {\bf Adversary's capability.}
Apart from deceiving SRSs, adversarial perturbation are required to be imperceptible to human hearings.
% Thus, the adversary is only allowed to perturb benign voices under some constraint.
Thus, %the adversary is not permitted to arbitrarily manipulate the perturbation.
% To achieve imperceptibility, the adversary can only make small changes to the benign voices.
% In this work, we adopt $L_\infty$ norm to quantify the magnitude of the perturbation, under which the adversary is allowed to add a small perturbation measured by this norm.
in this work, we adopt $L_\infty$ norm to quantify the magnitude of the perturbation and set an upper bound for this norm, the same as many prior works~\cite{DBLP:journals/corr/abs-1711-03280, abs-1801-03339, li2020adversarial,jati2021adversarial, zhang2021attack,chen2019real}.
The adversary is only allowed to add a perturbation within the upper bound to benign voices.
We also assume that the adversary can launch digital domain attack, i.e.,
feeding crafted adversarial voices in the form of audio file to the SRS directly via exposed API.
Over-the-air attack, where the adversarial voices are played by loudspeakers, then transmitted in the air channel and finally recorded by microphones, is out of the scope of this work. Under digital domain attack, the adversary does not need to take into account ambient and hardware noises accrued in over-the-air attack which would destroy the effectiveness of adversarial voices.
This assumption is practical and realistic given that commercial SRSs (e.g., Microsoft Azure~\cite{microsoft-azure-vpr} and SpeakIn~\cite{SpeakIn}) provide their API to the public to access their services.
% \chengk{TO DO: over-the-line}

% \subsubsection{Adversary's Knowledge}
% \subsection{Adversary's Knowledge}
\smallskip\noindent {\bf Adversary's knowledge.} 
% An adversary can own different levels of knowledge about the SR model under attack and the deployed defense.
% Knowledge about SR models ranges from detailed information of the victim model, including architecture and parameters, i.e., white-box attack, to can only acquiring the model's outputs (decision and/or scores) by providing some inputs, i.e., black-box attack.
% As for the deployed defense, the adversary may be
% % unaware of it (or has no access to it),
% unaware of it,
% or has full knowledge of it, including its implementation detail and concrete values for any tunable parameter.
% In the former case, the adversary craft adversarial voices without consideration for the defense, i.e., non-adaptive attack.
% For the latter, in contrast, the adversary makes his best to break the model and defense simultaneously, i.e., adaptive attack.
% % Under adaptive attack, the adversary make his best to bypass the defense.
% Different combinations of knowledge about SR models and deployed defenses leads to four attack scenarios considered in this work, i.e., white-box non-adaptive, black-box non-adaptive, white-box adaptive and black-box adaptive attacks.
An adversary may own different levels of knowledge about the SRS under attack,
from white-box access to model structure and parameters,
to black-box access to model outputs (decisions and/or scores).
White-box attack relies on detailed information of the victim model,
including internal architecture and learned parameters.
Thus, a white-box attack adversary can easily and precisely computes
the gradient of the loss w.r.t. the input by backpropagation.
In contrast, black-box attack assumes no knowledge about the model
but can access the target model as an oracle, i.e.,
providing a series of carefully crafted inputs to the model and observing its outputs.
As for the deployed defense, the adversary may be
unaware of it,
or has complete knowledge of it, including its implementation detail and concrete values for any tunable parameter.
In the former case, the adversary craft adversarial voices without considering the defense, i.e., non-adaptive attacks.
In the latter case,, the adversary makes his best to break the model and defense simultaneously, i.e., adaptive attacks.
Combinations of knowledge about SRS and deployed defenses lead to four attack scenarios considered in this work,
i.e., white-box non-adaptive, black-box non-adaptive, white-box adaptive and black-box adaptive attacks.

% \smallskip\noindent {\bf Knowledge about SR models.}

% \smallskip\noindent {\bf Knowledge about defenses.}

